Adaptive Artificial Time Delay Control for Robotic Systems

Artificial time delay controller was conceptualised for nonlinear systems to reduce dependency on precise system modelling unlike the conventional adaptive and robust control strategies. In this approach unknown dynamics is compensated by using input and state measurements collected at immediate past time instant (i.e., artificially delayed). The advantage of this kind of approach lies in its simplicity and ease of implementation. However, the applications of artificial time delay controllers in robotics, which are also robust against unknown state-dependent uncertainty, are still missing at large. This thesis presents the study of this control approach toward two important classes of robotic systems, namely a fully actuated bipedal walking robot and an underactuated quadrotor system. In the first work, we explore the idea of a unified control design instead of multiple controllers for different walking phases in adaptive bipedal walking control while bypassing computing constraint forces, since they often lead to complex designs. The second work focuses on quadrotors employed for applications such as payload delivery, inspection and search-and-rescue. The effectiveness of this controller is validated using experimental results.

==> 04_Quadrotor.tex <==
\chapter{Adaptive Artificial Time Delay Control for Quadrotors under State-dependent Unknown Dynamics}
\label{quad_chap}

The simplicity in implementation and the significantly low computation burden helped TDE-based methods to find remarkable acceptance in the control literature of robotics in the past decade \cite{Ref:jin2017model,Ref:roy2017adaptive, pi2019adaptive, brahmi2018adaptive, lee2019adaptive, roy2017adaptive,  lim2019delayed, roy2020new, mukherjee2019double, roy2017toward, roy2015robust, roy2017adaptive, mukherjee2021maneuvering} including in quadrotors \cite{lee2012experimental, wang2016model, dhadekar2021robust}, showing improved performances compared to conventional methods of robust and adaptive control. Yet, a formal stability analysis of TDE-controlled quadrotors with state-dependent uncertainities is missing. Therefore, a relevant question arises whether \textit{the existing TDE methods can tackle the unknown state-dependent uncertainties in quadrotors}, as, left unattended, such uncertainties can cause instability \cite{kocer2018centralized}. Unfortunately, the TDE methods for quadrotors \cite{lee2012experimental, wang2016model, dhadekar2021robust} (and relevant references therein) rely on the assumption of a priori bounded approximation error (a.k.a. \textit{TDE} error), which is quite common in TDE literature \cite{ Ref:jin2017model,Ref:roy2017adaptive, pi2019adaptive, lee2019adaptive, brahmi2018adaptive, lim2019delayed, mukherjee2019double, roy2017toward, roy2015robust, roy2017adaptive, mukherjee2021maneuvering} and hence, these methods are conservative for quadrotors to negotiate state-dependent uncertainties (please refer to Remark 4 later). Further, being an underactuated system, the adaptive TDE works \cite{Ref:jin2017model,Ref:roy2017adaptive, pi2019adaptive, lee2019adaptive, brahmi2018adaptive, roy2020new} are not directly applicable to a quadrotor. 

In light of the above discussions, artificial delay based adaptive control for quadrotors, which is also robust against \textit{unknown state-dependent uncertainty} is still missing. In this direction, this work has the following major contributions:

\begin{itemize}
\item The proposed adaptive TDE method for a quadrotor system, to the best of the authors' knowledge, is a first of its kind, because the existing TDE methods for quadrotors \cite{lee2012experimental, wang2016model, dhadekar2021robust} are non-adaptive solutions.
    \item Unlike the existing adaptive TDE solutions \cite{Ref:jin2017model,Ref:roy2017adaptive, pi2019adaptive, brahmi2018adaptive, lee2019adaptive}, the proposed adaptive TDE method can provide \emph{robustness} (hence termed as adaptive-robust TDE, ARTDE) against state-dependent unmodelled dynamics. 
    \item The closed-loop system stability is established analytically. Further, experimental results suggest significant improvement in tracking accuracy for the proposed method compared to the state of the art.
\end{itemize}

The rest of the chapter is organised as follows: Section 3.2 describes the dynamics of quadrotor;
Section 3.3 details the proposed control framework, while corresponding stability analysis is provided
in Section 3.4; comparative simulation results are provided in Section 3.5.


\section{Quadrotor System Dynamics}
\begin{figure}[!h]
    \includegraphics[width=2in, height=2in]{images/quadrotor/drone_model_BodyWorld.png}
    \centering
    \caption{Schematic of a quadrotor and the coordinate frames.}
    \label{fig:quad_axis}
\end{figure}
	The well established Euler-Lagrangian system dynamics of a quadrotor model is given by \cite{bialy2013lyapunov}
	\begin{subequations}\label{dyn}
	\begin{align}	
	&	m \ddot{p}(t) + G +  d_p(p(t), \dot{p}(t),t) = \tau_p(t), \label{p_tau} \\
	&	J (q(t))\ddot{q}(t) + C_q(q(t),\dot{q}(t))\dot{q}(t) +  d_q(q,\dot{q},t) = \tau_q(t), \label{q_tau} \\
	&	\tau_p (t) = R_B^W (q)U(t), \label{tau_conv}
	\end{align}
	\end{subequations}
	where (\ref{p_tau}) and (\ref{q_tau}) are the position dynamics and the attitude dynamics, respectively; (\ref{tau_conv}) converts the input vector $\tau_p \in \mathbb{R}^3$ in Earth-fixed frame to $U\triangleq
	\begin{bmatrix}
	0 & 0 & u_1
	\end{bmatrix}^T\in \mathbb{R}^3$ in body-fixed frame via the rotational matrix $R_B^W$ given by
	\begin{align}
	R_B^W =
	\begin{bmatrix}
	c_{\psi}c_{\theta} & c_{\psi}s_{\theta}s_{\phi} - s_{\psi}c_{\phi} & c_{\psi}s_{\theta}c_{\phi} + s_{\psi}s_{\phi} \\
	s_{\psi}c_{\theta} & s_{\psi}s_{\theta}s_{\phi} + c_{\psi}c_{\phi} & s_{\psi}s_{\theta}c_{\phi} - c_{\psi}s_{\phi} \\
	-s_{\theta} & s_{\phi}c_{\theta} & c_{\theta}c_{\phi}
	\end{bmatrix}, \label{rot_matrix}
	\end{align}
	where $c_{(\cdot)} , s_{(\cdot)}$ are abbreviations for $\cos{(\cdot)} , \sin{(\cdot)}$ respectively. Various other symbols in (\ref{dyn}) are described as follows: the mass and inertia matrix are represented by $m \in \mathbb{R}^{+}$ and $J(q) \in \mathbb{R}^{3 \times 3}$ respectively; the center-of-mass of the quadrotor is denoted by the position vector $p\triangleq
	\begin{bmatrix}
	x & y & z
	\end{bmatrix}^T \in\mathbb{R}^3$; the orientation/attitude (roll, pitch, yaw angles respectively) is denoted via $q\triangleq \begin{bmatrix}
	\phi & \theta & \psi
	\end{bmatrix}^T\in \mathbb{R}^3$; $G\triangleq
	\begin{bmatrix}
	0 & 0 & mg
	\end{bmatrix}^T\in \mathbb{R}^3$ denotes the gravitational force vector with gravitational constant $g$; $C_q(q, \dot{q}) \in \mathbb{R}^{3 \times3}$ is the Coriolis matrix; the unmodelled disturbances, which can be both state and time dependent, are denoted by $d_p$ and $d_q$; $\tau_q \triangleq 
	\begin{bmatrix}
	u_2 & u_3 & u_4
	\end{bmatrix}^T\in\mathbb{R}^3$ are the control inputs for roll, pitch and yaw; %$\tau_p \in \mathbb{R}^3$ is the generalized control input for position tracking in Earth-fixed frame, with $U\triangleq
	%\begin{bmatrix}
	%0 & 0 & u_1
	%\end{bmatrix}^T\in \mathbb{R}^3$ being the force vector in body-fixed frame and $R_B^W \in\mathbb{R}^{3\times3}$ is the $Z$-$Y$-$X$ Euler angle rotation matrix from the body-fixed to the Earth-fixed frame,  
	
%	From the standard Euler-Lagrange mechanics, the following property holds :
	
\textbf{Property 1.} Standard Euler-Lagrange mechanics implies the inertia matrix $J (q)$ is uniformly positive definite $\forall q$ \cite{bialy2013lyapunov}. % and $ \exists \underline{j},\overline{j} \in{R}^{+}$ such that $0 \leq \underline{j}I \leq J(q) \leq \overline{j}I$. 

In the following, we highlight the available system parametric knowledge for control design:
\begin{assumption}
The exact knowledge of $m,J$ is not available, and only some upper bounds are known (cf. Remark 6 later); meanwhile, the system dynamics term $C_q(q,\dot{q})$, unmodelled (possibly state-dependent) dynamics $d_p,d_q$ and their bounds are unknown for control design. %The terms $d_p,d_q$ can have state-dependency, and hence cannot be bounded a priori.
\end{assumption}
\begin{remark}[Validity of assumption 1]
In practice, maximum allowable payload is always known; hence, a priori upper bound knowledge of $m$ and $J$ is plausible for control design, while handling other unknown state-dependent dynamics terms is a control challenge solved in this work. 
\end{remark}
%\begin{remark}[Position and attitude tracking co-design]\label{rem_co}
%Tracking control problem of quadrotors can be broadly classified under two categories: (i) reduced-order model based design (cf. \cite{nicol2011robust, dydek2012adaptive, ha2014passivity, mofid2018adaptive}) and (ii) position and attitude tracking co-design (cf. \cite{bialy2013lyapunov, mellinger2011minimum}). Control designs relying on the first category ignore the non-actuated $(x,y)$ dynamics and define the control problem as tracking of only the actuated degrees-of-freedom (DoF) i.e. of $z$ and $(\phi, \theta ,\psi)$. Such approach is generally termed as `collocated design' in the literature of underactuated systems (cf. \cite{roy2020towards}). The second category relies on co-designing position and attitude tracking controller for the six DoF dynamics (\ref{p_tau})-(\ref{q_tau}). 
%\end{remark}

%In this work, we shall follow the co-design approach as the reduced-order based approach is conservative for relying on a priori boundedness of $(x,y)$ dynamics. 
%We further take the following standard assumption:


\begin{assumption}[\cite{ mellinger2011minimum, sankaranarayanan2020aerial}]\label{assum_des}
The desired position $p_d  \triangleq
	\begin{bmatrix}
	x_d  & y_d  & z_d
	\end{bmatrix}^T$ and yaw trajectories $\psi _d $ are designed such that they are smooth and bounded. %Further, it is assumed that the following inequality holds for all time: $ - \frac{\pi}{2} < (\phi_d, \theta_d) < \frac{\pi}{2}$ radians.
\end{assumption}
\begin{remark}[Desired roll and pitch]
As standard in literature \cite{mellinger2011minimum}, the desired roll ($\phi_d$) and pitch $(\theta_d$) angle trajectories are computed using $\tau_p$ and $\psi_d$. % (cf. ) and it is discussed later (cf. Sect. III.B).
\end{remark}


\section{Proposed Controller Design and Analysis}
%
%The objective of the controller is to guarantee that $p (t)$ and $\psi (t)$ to track any desired trajectory provided  $p_d (t) \triangleq
%	\begin{bmatrix}
%	x_d (t) & y_d (t) & z_d (t)
%	\end{bmatrix}^T\in{\mathbb{R}^3}$ and $\psi (t) \in{\mathbb{R}}$ exist and are bounded. The subsequent control development and analysis is based on the common assumption that the desired trajectories are sufficiently smooth, bounded, and are chosen such that the following inequality holds for all time: $ - \frac{\pi}{2} < (\phi, \theta) < \frac{\pi}{2}$ radians.

\subsection{Control Problem and Objective} Under Property 1 and Assumption 1, the aim is to design an adaptive robust TDE (ARTDE) controller for quadrotors to track a desired trajectory (cf. Assumption 2). 

Since the aim is to design controller for the complete six degrees-of-freedom quadrotor dynamics, the standard position and attitude co-design method is followed (cf. \cite{ mellinger2011minimum}) instead of the reduced-order model one (cf. \cite{ dydek2012adaptive, mofid2018adaptive}). Such approach (cf. Fig. \ref{fig:block_dia} later) relies on simultaneous design of an outer loop controller for (\ref{p_tau}) and of an inner loop controller for (\ref{q_tau}) as described in the following subsections. % elaborate the proposed ARTDE framework along with stability analysis. % to thecontrol problem is solved
 \subsection{Outer Loop Controller}
Let the position tracking error be defined as ${e_p}(t)={p}^d(t)-{p}(t)$. The variable dependency will be removed subsequently for brevity whenever it is obvious.
% \begin{align}
%     e_p &= p - p_d \label{p_err}
%\end{align} 
%Before presenting the outer loop controller, 
The position dynamics (\ref{p_tau}) is re-arranged by introducing a constant ${\bar {m}}$ as
\begin{align} 
&{\bar{m}\ddot {p}} + {{N_p}}({{p}},{{\dot { p}},\ddot{ p}}) = {\boldsymbol {\tau}_p }, \label{robotdynamics2}\\
%\end{equation}
%\begin{equation} 
\text{with}~~~~&{{N_p}}({{p}},{{\dot { p}},\ddot{ p}}) = ({{m}} - {\bar {m}}){\ddot {p}} +  G + {d_p}\nonumber
\end{align}
and the selection of ${\bar {m}}$ is discussed later (cf. Remark \ref{rem_up}). Note that, $N_p$ contains unknown state-dependent (via $(p, \dot{p})$) dynamics $d_p$ (cf. Assumption 1) and hence, it is not a priori bounded.

The control input $\boldsymbol{\tau}_p$ is proposed as
\begin{subequations}\label{tau}
\begin{align}
\boldsymbol{\tau}_p &=\bar{m} u_p+\hat{ N}_p({{p}},{{\dot {p}},\ddot{p}}), \label{input}\\
{u}_p &= {u_p}_0+\boldsymbol\Delta u_p,~%\label{tarc input}\\
{u_p}_0 =\ddot{p}^d +  K_{1p}\dot{e}_p + K_{2p}  e_p, \label{aux}
\end{align}
\end{subequations}
where $K_{1p}, K_{2p} \in {R}^{3 \times 3}$ are two user-defined positive definite matrices; $\boldsymbol\Delta u_p$ is the adaptive control term responsible to tackle uncertainties in position dynamics and it will be designed later; $\hat{ N}_p$ is the estimation of $N_p$ derived from the past state and input data as
\begin{equation}\label{approx_p}
{\hat{ N}_p( p,\dot{ p} , \ddot{ p})\cong}N_p( p_L,\dot{ p}_L,\ddot{p}_L)=\boldsymbol(\tau_p)_L-\bar{ m}\ddot{ p}_L,
\end{equation}
where $L>0$ is a small time delay which and its choice is discussed later. The notation $(\cdot)_L$ is defined in Sect. I.
\begin{remark}[Artificial time delay]\label{rem_tde}
The estimation of uncertainty as in (\ref{approx_p}) is based on intentionally (or artificially) introducing a time delay (a.k.a TDE) in the form of past data; some literature (cf. \cite{ Ref:jin2017model,Ref:roy2017adaptive, pi2019adaptive, lee2019adaptive, brahmi2018adaptive, lim2019delayed} and referenced therein) terms this mechanism as artificial time delay based design.
\end{remark}

Substituting (\ref{input}) into (\ref{robotdynamics2}), one obtains
\begin{align}
\ddot{e}_p& =- K_{1p}\dot{ e}_p- K_{2p} e_p+\boldsymbol \sigma_p -\boldsymbol\Delta u_p , \label{error dyn delayed 2}
\end{align}
where $\boldsymbol\sigma_p={{\frac{1}{\bar{m}}}}({ N_p}-{\hat{ N}_p})$ is the \textit{estimation error originating from (\ref{approx_p})} and it is termed as the \textit{TDE error}.

%The adaptive control term $\Delta \mathbf u_p$ is designed based on the structure of the upper bound of TDE error $\boldsymbol\sigma_p$. Therefore,
In the following, we first derive the upper bound structure of $|| \boldsymbol\sigma_p ||$, based on which the adaptive control term $\Delta \mathbf u_p$ is designed  subsequently. % design the proposed adaptive law.

\subsubsection{Upper bound structure of $||\boldsymbol \sigma_p||$} \label{sec bound}
From (\ref{robotdynamics2}) and (\ref{error dyn delayed 2}), once can derive the following:
\begin{align}
\hat{N}_p&=(N_p)_L=[{{m}}({{p}_L}) - {\bar { m}}]{\ddot { p}_L} + G_L + (d_p)_L ,\label{sig 2} \\%(\mathbf q,\dot{\mathbf q}) \\
\boldsymbol \sigma_p&=\ddot{ p}- u_p. \label{sig 1} 
\end{align}
Using (\ref{sig 2}), the control input $\boldsymbol \tau_p$ in  (\ref{input}) can be rewritten as
\begin{align}
\boldsymbol {\tau}_p &= \bar{m} u_p+[{ {m}}({{p}_L}) - {\bar {m}}]{\ddot { p}_L} +  G_L + (d_p)_L. \label{tau new}
\end{align}
Multiplying both sides of (\ref{sig 1}) with $m$ and using (\ref{robotdynamics2}) and (\ref{tau new}) we have
\begin{align}
&{m} \boldsymbol \sigma_p  = \boldsymbol {\tau}_p  - N_p-{m}{u_p} \nonumber \\
& = \bar{m}  u_p+[{{m}}({{p}_L}) - {\bar { m}}]{\ddot {p}_L} + G_L + (d_p)_L -N_p -{m}{u_p}. \label{sig 3}
\end{align}
Using (\ref{error dyn delayed 2}) we have
\begin{align}
\ddot{{p}}_L&=\ddot{{p}}^d_L-\ddot{{e}}_L =\ddot{{p}}^d_L +K_p\boldsymbol \xi_L-\boldsymbol \sigma_L+(\boldsymbol\Delta  {u_p})_L,\label{sig 4}
\end{align}
where $K_p \triangleq [K_{1p} ~ K_{2p}]$, $\xi_L= [
{ e_L}^T~
\dot{e_L}^T]^T$. Substituting (\ref{sig 4}) into (\ref{sig 3}), and after re-arrangement yields
\begin{align}
\boldsymbol \sigma_p &= \underbrace{m^{-1}\bar{{m}}(\boldsymbol \Delta u_p- \boldsymbol (\Delta  u_p)_L)}_{\boldsymbol \chi_1}+\underbrace{m^{-1}({m}_L\boldsymbol (\Delta u_p)_L-{m}\boldsymbol (\Delta u_p)_L)}_{\boldsymbol \chi_2} \nonumber\\
&+\underbrace{m^{-1}\lbrace (\bar{{m}} - {m})\ddot{{p}}^d-({m} - {m}_L)\ddot{{p}}^d_L+ G_L + (d_p)_L - G - d_p \rbrace }_{\boldsymbol \chi_3} \nonumber\\
%\end{align}
%\begin{align}
& +\underbrace{m^{-1}({m}_L-\bar{{m}}){K}_p\boldsymbol \xi_L}_{\boldsymbol \chi_4}-\underbrace{m^{-1}({m}_L-\bar{{m}})\boldsymbol \sigma_L}_{\boldsymbol \chi_5} \nonumber\\
&+\underbrace{(\bar{{m}}/m-1){K}_p\boldsymbol \xi_p}_{\boldsymbol \chi_6}. \label{sig 5}
\end{align}
%Further, $\boldsymbol \Delta \dot{\mathbf u}$ is continuous and the EL system (\ref{sys}) is at least $\mathcal{C}^1$ continuous. Consider the system to be locally Lipschitz continuous $\forall \theta \in [-L ~ 0]$. 
Using the relation $(\cdot)_L= %\psi(t-L)=
(\cdot)(t)-\int_{-L}^0 {\frac{\mathrm{d}}{\mathrm{d}\theta}(\cdot)}(t+\theta)\mathrm{d}\theta$ and the fact that integration of any continuous function over a finite interval (here $-L$ to $0$) is always finite \cite{roy2021artificial}, the following conditions hold for unknown constants $\delta_i$, $i=1, \cdots,5$:
\begin{align}
&|| {\boldsymbol \chi_1} ||=|| \frac{1}{m}\bar{{m}} \int_{-L}^{0} \frac{{d}}{{d}\theta}\boldsymbol \Delta { u_p}(t+\theta) {d}\theta || \leq \delta_1 \label{sig 6}\\
&|| {\boldsymbol \chi_2} ||=||\frac{1}{m}\hspace{-.1cm} \int_{-L}^{0} \frac{{d}}{{d}\theta}{m}(t+\theta)\boldsymbol \Delta {u}_p(t+\theta) {d}\theta || \leq \delta_2\\
&|| {\boldsymbol \chi_3} ||=||\frac{1}{m}\lbrace (\bar{{m}} -m)\ddot{{p}}^d-({m}-{m}_L)\ddot{{p}}^d_L \nonumber\\
&\qquad \qquad \qquad  G_L + (d_p)_L -G -d_p \rbrace ||\leq \delta_3 \\
&|| {\boldsymbol \chi_4} ||=|| \frac{1}{m} \int_{-L}^{0} \frac{{d}}{{d}\theta}({m}(t+\theta)-\bar{{m}}){K}_p\boldsymbol \xi_p(t+\theta) {d}\theta  \nonumber \\
& \qquad \qquad +(\bar{{m}}/m-1){K}_p\boldsymbol \xi_p  ||\leq || E_p  K_p ||  ||\boldsymbol \xi_p || +\delta_4 \\
&|| {\boldsymbol \chi_5} ||=|| E_p \boldsymbol \sigma_p +  \frac{1}{m} \int_{-L}^{0} \frac{{d}}{{d}\theta}\lbrace({m}(t+\theta)-\bar{{m}}) \boldsymbol \sigma_p (t+\theta) \rbrace {d}\theta || \nonumber \\
& \qquad \leq ||{ E_p}|| ||\boldsymbol \sigma_p ||  + \delta_5  \label{del_5}\\
&|| {\boldsymbol \chi_6} ||= || (\bar{{m}}/m-1){K}_p\boldsymbol \xi_p || \leq || {E_p}{K}_p|| ||\boldsymbol \xi_p||, \label{sig 7}
\end{align} 
and the following holds
\begin{equation}
   | E_p |= | 1 -\bar{m}/m | <1. \label{E_p} 
\end{equation}
Using (\ref{sig 5}) and (\ref{sig 6})-(\ref{sig 7}), one derives
\begin{align}
 \lVert \boldsymbol \sigma_p \rVert &\leq \beta_{0p} + \beta_{1p} \lVert\boldsymbol \xi_p \rVert, \label{sig bound} \\
 \text{where}~ &\beta_{0p}=\frac{\sum_{i=1}^{5}\delta_i}{1-| E_p |}, ~ \beta_{1p}=\frac{2 \lVert E_p  K_p \rVert  }{1-| E_p|} \label{beta}.
\end{align}

%with \begin{align}
%     ~\alpha_{qi} > 0~ \label{q_init_K}
%\end{align}
\subsubsection{Designing $\Delta u_p$} \label{sec gain}
The term $\boldsymbol\Delta u_p$ is designed as
\begin{align}
&\boldsymbol\Delta {{u}}_p =\alpha_p c_p ({s_p}/{||s_p||}),  \label{delta u2_p} %\text{sig}({s_p},\epsilon_p)
\end{align}
where ${s_p=B}^T{U_p}\xi_p$, $\xi_p= \begin{bmatrix}
{ e_p}^T&
\dot{e_p}^T
\end{bmatrix}^T$ and $U_p$ is the solution of the Lyapunov equation ${A_p}^TU_p+{U_p}{A_p}=-Q_p$ for some ${Q_p>0}$, where $  A_p=\begin{bmatrix}
{0} & {I} \\
-{K}_{2p} & -{K}_{1p}
\end{bmatrix}$, ${B}=\begin{bmatrix}
{0}\\
{I}
\end{bmatrix}$; $\alpha_p \in \mathbb{R}^{+}$ is a user-defined scalar; ${c_p}$ is the switching gain which provides robustness against the TDE error and % and $\text{sig}({s,\epsilon})$ is a smooth sigmoid function defined as $\text{sig}({s},\epsilon) \triangleq {{s}}/{\sqrt{|| {s}||^2+\epsilon}}.$
%Here, $\epsilon_p$ is a small positive scalar used to avoid chattering.
it is constructed from the upper bound structure of $||\boldsymbol \sigma_p ||$ as
\begin{align}
c_p=\hat{\beta}_{0p}+\hat{\beta}_{1p} ||\boldsymbol \xi_p || , \label{sw_gain_p} %+\hat{\beta}_2)
\end{align}
where $\hat{\beta}_{0p}, \hat{\beta}_{1p}$ are the estimates of $\beta_{0p}, \beta_{1p}$, respectively and they are evaluated as follows: %using the following adaptive law:
\begin{align}
\dot{\hat{\beta}}_{ip} =
  \begin{cases}
     \lVert\boldsymbol \xi_p \rVert^i \lVert  s_p \rVert,       &  {\text{if} ~ \text{any}~\hat{\beta}_{ip} \leq \underline{\beta}_{ip} ~ \text{or} ~{s}_p^T \dot{{s}}_p >0} \\
    -  \lVert\boldsymbol \xi_p \rVert^i \lVert  s_p \rVert,       & {\text{if} ~ {s}_p^T \dot{{s}}_p  \leq 0 ~\text{and all}~  \hat{\beta}_{ip} > \underline{\beta}_{ip} }
  \end{cases}, \label{ATRC_p} 
\end{align}
\noindent with $\hat{\beta}_{ip}(0) \geq \underline{\beta}_{ip} >0$, $i=0,1$ are user-defined scalars. Combining (\ref{tau}), (\ref{sig bound}) and (\ref{ATRC_p}), we have
\begin{equation}\label{theproposedcontrollaw_p}
\begin{split}
{\boldsymbol{\tau_p }} = & \underbrace {({\boldsymbol{\tau }_p)_L} - {\bar{m}}{{{\ddot { p}}}_L}}_{{\text{TDE~part}}}+\underbrace {{\bar{ m}}({{{\ddot { p}}}^d} + K_{1p}{\dot e}_p + K_{2p}{e_p})}_{{\text{Desired~dynamics~injection~part}}}+\underbrace { {\bar{ m}} c_p (s_p/||s_p||) .}_{{\text{Adaptive-robust~control~part}}} %\text{sig}({{s_p}},\epsilon_p)
\end{split}
\end{equation}
Eventually, $U$ is applied to the system using $\tau_p$ as in (\ref{tau_conv}). % ($R^W_B$ is invertible rotational matrix), giving non-zero input only in $z$ direction.
\subsection{Inner Loop Controller}
%For designing the inner loop controller, the desired roll ($\phi_d$) and pitch ($\theta_d$) angles are computed using $\tau_p$ and $\psi_d (t)$ \cite{mellinger2011minimum} (cf. Remark 2). % (the details are omitted here due to lack of space). 
The orientation/attitude error is defined as \cite{mellinger2011minimum}
\begin{align}
    e_q &= {((R_d)^T R_B^W - (R_B^W)^T R_d)}^{v} \label{q_err} \\ \nonumber
    \dot{e}_q & = \dot{q} - R_d^T R_B^W \dot{q}_d
\end{align}
where $R_d$ is the rotation matrix as in (\ref{rot_matrix}) evaluated at ($\phi_d, \theta_d, \psi_d$) and $(.)^v$ is the \textit{vee} map converting elements of $SO(3)$ to $\in{\mathbb{R}^3}$ \cite{mellinger2011minimum} ($\phi_d, \theta_d$ are generated as per Remark 2).

Introducing a constant matrix $\bar{J}$ (cf. Remark \ref{rem_up} for its choice), the attitude dynamics (\ref{q_tau}) is re-arranged as 
\begin{align} 
&{\bar{J}\ddot {q}} + {{N_q}}({{q}},{{\dot { q}},\ddot{q}}) = {\boldsymbol {\tau}_q } \label{sys_q},\\
%\end{equation}
%\begin{equation} 
\text{with}~~~~&{{N_q}}({{q}},{{\dot { q}},\ddot{ q}}) = [{{J}} - {\bar {J}}]{\ddot {q}} +  C_q{\dot { q}} + {d_q}.
\end{align}
The control input $\boldsymbol{\tau}_q$ is designed as
\begin{subequations}\label{tau_q}
\begin{align}
\boldsymbol{\tau}_q &=\bar{J} u_q+\hat{ N}_q({{q}},{{\dot {q}},\ddot{q}}), \label{input_q}\\
{u}_q &= {u_q}_0+\boldsymbol\Delta u_q, ~ %\label{tarc input_q}\\
{u_q}_0 =\ddot{q}^d +  K_{1q}\dot{e}_q + K_{2q}  e_q, \label{aux_q}
\end{align}
\end{subequations}
where $K_{1q}, K_{2q} \in {R}^{3 \times 3}$ are two user-defined positive definite matrices; the adaptive control term $\boldsymbol\Delta u_q$, used for tackling uncertainties in attitude dynamics, would be designed later; $\hat{ N}_q$ is the estimation of $N_q$ computed via TDE as
\begin{equation}\label{approx_q}
{\hat{ N}_q( q,\dot{ q} , \ddot{ q})\cong}N_q( q_L,\dot{ q}_L,\ddot{q}_L)=\boldsymbol(\tau_q)_L-\bar{ J}\ddot{ q}_L.
\end{equation}
Substituting (\ref{input_q}) into (\ref{sys_q}), we obtain the error dynamics as
\begin{align}
\ddot{e}_q& =- K_{1q}\dot{ e}_q- K_{2q} e_q+\boldsymbol \sigma_q- \boldsymbol\Delta u_q, \label{error dyn delayed 2_q}
\end{align}
where $\boldsymbol\sigma_q={\bar{J}}^{-1}({ N_q}-{\hat{N_q}})$ represents the attitude \textit{TDE error}.

\subsubsection{Upper bound structure of $||\boldsymbol \sigma_q||$}The upper bound structure for $||\sigma_q||$ can be derived in a similar way to that of $||\sigma_p||$ in Sect. \ref{sec bound} as (omitted due to lack of space) 
%and it is found as
\begin{align}
 \lVert \boldsymbol \sigma_q \rVert &\leq \beta_{0q} + \beta_{1q} \lVert\boldsymbol \xi_q \rVert, \label{sig bound_q} \\
 \text{where}~ &\beta_{0q}=\frac{\sum_{i=1}^{5}\bar{\delta}_i}{1-\lVert E_q \rVert}, ~ \beta_{1q}=\frac{2 \lVert E_q  K_{q} \rVert  }{1-\lVert E_q\rVert}, K_q \triangleq [K_{1q} ~ K_{2q}] \nonumber 
\end{align}
where $\bar{\delta}_i$ are unknown constants and the following holds
\begin{equation}
   || E_q ||= ||J^{-1}\bar{J}-I|| < 1. \label{E_q} 
\end{equation}
\subsubsection{Designing $\Delta u_q$} The term $\boldsymbol\Delta u_q$ is designed as
\begin{align}
&\boldsymbol\Delta {{u}}_q =\alpha_q c_q({s_q}/{||s_q|| }),  \label{delta u2} %\text{sig}({s_p},\epsilon_p)
\end{align}
where ${s_q=B}^T{U_q}\xi_q$, $\xi_q= \begin{bmatrix}
{ e_q}^T&
\dot{e_q}^T
\end{bmatrix}^T$ and $U_q$ is the solution of the Lyapunov equation ${A_q}^TU_q+{U_q}{A_q}=-Q_q$ for some ${Q_q>0}$, where $  A_q=\begin{bmatrix}
{0} & {I} \\
-{K}_{2q} & -{K}_{1q}
\end{bmatrix}$, ${B}=\begin{bmatrix}
{0}\\
{I}
\end{bmatrix}$; $\alpha_q \in \mathbb{R}^{+}$ is a user-defined scalar; ${c_q} $ is the adaptive gain designed as
\begin{align}
c_q=\hat{\beta}_{0q}+\hat{\beta}_{1q} ||\boldsymbol \xi_q || , \label{sw_gain_q} %+\hat{\beta}_2)
\end{align}
where $\hat{\beta}_{0q}, \hat{\beta}_{1q}$ are the estimates of $\beta_{0q}, \beta_{1q} \in \mathbb{R}^{+}$, respectively. % and 
The gains are evaluated as follows: %using the following adaptive law:
\begin{align}
\dot{\hat{\beta}}_{iq} =
  \begin{cases}
   \lVert\boldsymbol \xi_q \rVert^i \lVert  s_q \rVert,       &  {\text{if} ~ \text{any}~\hat{\beta}_{iq} \leq \underline{\beta}_{iq} ~ \text{or} ~{s}_q^T \dot{{s}}_q >0} \\
    -  \lVert\boldsymbol \xi_q \rVert^i \lVert  s_q \rVert,       & {\text{if} ~ {s}_q^T \dot{{s}}_q  \leq 0 ~\text{and all}~  \hat{\beta}_{iq} > \underline{\beta}_{iq} }
  \end{cases}, \label{ATRC_q} 
\end{align}
\noindent with $\hat{\beta}_{iq}(0) \geq \underline{\beta}_{iq} >0$, $i=0,1$ are user-defined scalars. Finally, the inner loop control becomes
\begin{equation}\label{theproposedcontrollaw_q}
\begin{split}
{\boldsymbol{\tau_q }} = & \underbrace {({\boldsymbol{\tau }_q)_L} - {\bar{J}}{{{\ddot { q}}}_L}}_{{\text{TDE~part}}}+\underbrace {{\bar{ J}}({{{\ddot { q}}}^d} + {{{K_1}}_q}{\dot { e_q}} + {{{K_2}}_q}{{e_q}})}_{{\text{Desired~dynamics~injection~part}}}
+\underbrace {{\bar{ J}} c_q (s_q/||s_q||) .}_{{\text{Adaptive-robust~control~part}}} %
\end{split}
\end{equation}
Figure \ref{fig:block_dia} depicts the overall proposed control framework.
\begin{figure}[!h]
    \centering
    \includegraphics[width=1\linewidth]{images/quadrotor/block_diagram.png}
    \centering
    \caption{Block diagram of the proposed ARTDE control framework via the outer- and inner loop co-design approach.}
    \label{fig:block_dia}
\end{figure} 
\begin{remark}[State-dependent TDE error bound]\label{rem_new}
Note from (\ref{sig bound}) and (\ref{sig bound_q}) that the TDE errors $\boldsymbol \sigma_p, \boldsymbol \sigma_q$ depend on states via $\boldsymbol \xi_p, \boldsymbol \xi_p$ respectively and hence cannot be bounded a priori: for this reason, the standard TDE-based methods \cite{ Ref:jin2017model,Ref:roy2017adaptive, pi2019adaptive, brahmi2018adaptive, lim2019delayed} are not applicable for quadrotors as they rely on a priori bounded TDE error (i.e., they assume $\beta_{1p}=0$). ARTDE mainly differs from the state-of-the-art in the way its switching gain is adapted to tackle state-dependent uncertainty and the consequent stability analysis. %This work solves this issue. %Similar case can be noted for attitude dynamics (cf. (\ref{sig bound_q}) later). %Therefore, a new and suitable adaptive law $\Delta u_p$ is derived subsequently.
\end{remark}

\begin{remark}[Choice of $L$]
It can be noted from (\ref{sig 6})-(\ref{del_5}), that high value of time delay $L$ will lead to high values of $\delta_i$, i.e., larger TDE error: therefore, one needs to select the smallest possible $L$, which is usually selected as the sampling time of the low level micro-controller \cite{ Ref:jin2017model,Ref:roy2017adaptive, pi2019adaptive, brahmi2018adaptive, lee2019adaptive, lim2019delayed, lee2012experimental, wang2016model, dhadekar2021robust}.
\end{remark}
\begin{remark}[On the choice of $\bar{m}$ and $\bar{J}$]\label{rem_up}
From the upper bounds on $m$ and $J$ (cf. Assumption 1), one can always design $\bar{m}$ and $\bar{J}$ which satisfy (\ref{E}) and (\ref{E_q}) respectively, which is standard in TDE literature \cite{ Ref:jin2017model,Ref:roy2017adaptive, pi2019adaptive, lee2019adaptive, brahmi2018adaptive, lim2019delayed}: hence, we do not introduce any additional constraint. % while tackling the state-dependent TDE error.
%Note that the inner and outer loop design processes are coupled via $\tau_p$ and simultaneously affect the quadrotor system: this makes the proposed design a more realistic one compared to decoupled dynamics based approaches (cf. \cite{nicol2011robust, dydek2012adaptive, ha2014passivity, mofid2018adaptive}) or linearized and decoupled autopilot based designs (cf. \cite{fari2019addressing,yang2019software}).
\end{remark}


\begin{algorithm}[!h]

 \caption{ {Design steps of the proposed controller}}
 \vspace{0.2cm}
 
\textbf{Step 1 (Defining the outer-loop error variables):} Find $e_p$ via (\ref{robotdynamics2}); define gains ${K_P}_1, {K_P}_2$ and solve for $U_a$ from (\ref{sec gain}) to compute $s_p = B^T U_p\xi_p$. 

\textbf{Step 2 (Designing adaptive gains for outer-loop):} Using variables from Step 1, compute gain $c_p$ from (\ref{sw_gain_p}) using the adaptive laws (\ref{ATRC_p}). % which provide the gains to compensate for the uncertainties are designed based on the structure of the TDE error upper bound.

\textbf{Step 3 (Computing $\tau_p$ and $U$):} Select $\overline{m}$ from (\ref{E_p}); then, using results from Steps 1-2, compute outer-loop control input $\tau_p$ from (\ref{theproposedcontrollaw_p}) after designing gains ${K_P}_2, {K_D}_2$ and deriving $\hat{N}_p$ via TDE method (\ref{approx_p}). Compute $U$ from $\tau_p$ as per (\ref{tau_conv}).

\textbf{Step 4 (Defining the inner-loop error variables):} %Evaluate $\phi^d, \theta^d$ using $\tau_p$ and $\psi^d$ as per \cite{} and then,
Compute error variable $e_q, \dot{e}_q$ from (\ref{q_err}) and design gains ${K_P}_3, {K_D}_3$ to evaluate $U_q$ from (\ref{delta u2}) and compute $s_q = B^T U_q\xi_q$.

\textbf{Step 5 (Designing adaptive gains for inner-loop):} Using variables from Step 4 and adaptive laws (\ref{ATRC_q}), evaluate gain $c_q$ from (\ref{sw_gain_q}).

\textbf{Step 6 (Computing $\tau_q$):} Using results from Steps 4-5, compute inner-loop control input $\tau_q$ from (\ref{theproposedcontrollaw_q}) after deriving $\hat{N}_q$ from TDE method (\ref{approx_q}) and suitably choosing $\overline{J}$ from (\ref{E_q}).

\textbf{Step 7 (Control input to system):} Finally, apply $U$ and $\tau_q$ from Steps 3 and 6 respectively to the quadrotor. 
\vspace{0.2cm}
 \end{algorithm}

\subsection{Stability Analysis}
\begin{theorem}
Under Assumptions 1-2 and Property 1, the closed-loop trajectories of (\ref{robotdynamics2}) and (\ref{sys_q}) using the control laws (\ref{theproposedcontrollaw}), (\ref{theproposedcontrollaw_q}), the adaptive laws (\ref{ATRC_p}), (\ref{ATRC}) and design conditions (\ref{E}) and (\ref{E_q}), are Uniformly Ultimately Bounded (UUB).
\end{theorem}
\textit{Proof : }
The stability analysis of ARTDE is carried out using the following Lyapunov function candidate:
\begin{align}
V& = (1/2)(\boldsymbol \xi_p^T{U_{p}} \boldsymbol \xi_{p} + \boldsymbol \xi_{q}^T{U_{q}} \boldsymbol \xi_{q}) + \frac{1}{2} \sum_{i=0}^{1}{(\hat{\beta}_{i{p}}-\beta_{i{p}})^2}+(\hat{\beta}_{i{q}}-\beta_{i{q}})^2 \label{lyapunov1}
\end{align}
The error dynamics (\ref{error dyn delayed 2}) and (\ref{error dyn delayed 2_q}) can be written as
\begin{align}
\dot{\boldsymbol \xi}_p& =A_p \boldsymbol\xi_p+{B} (\boldsymbol\sigma_p-\boldsymbol\Delta  u_p),
\dot{\boldsymbol \xi}_q=A_q \boldsymbol\xi_p+{B} (\boldsymbol\sigma_q-\boldsymbol\Delta  u_q)\label{error dyn delayed_q}
\end{align}
Positive definiteness of $K_{ip}$ and $ K_{iq}$ $i=1,2$ guarantee that ${A}_p$ and $A_q$ are Hurwitz. The first condition in the adaptive laws (\ref{ATRC_p}), (\ref{ATRC}) reveal that gains $\hat{\beta}_{ip}$ and $\hat{\beta}_{iq}$ increase if they attempt to go below $\underline{\beta}_{ip} $ and $\underline{\beta}_{iq} $ respectively; this yields $\hat{\beta}_{ip}(t) \geq  \underline{\beta}_{ip} $, $\hat{\beta}_{iq}(t) \geq  \underline{\beta}_{iq} $ $\forall t \geq 0$ $\forall i=0,1$. Further, these adaptive laws enumerate the following four possible cases.

\textbf{Case (i):} Both $\dot{\hat{\beta}}_{ip}(t) >0, \dot{\hat{\beta}}_{iq}(t) >0 $ \\
Using the Lyapunov equations ${A}_p^T{U_p+U_pA_p=-Q_p}$, ${A}_q^T{U_q+U_q A_q=-Q_q}$, and the adaptive laws (\ref{ATRC_p}), (\ref{ATRC}) yield % the time derivative of (\ref{lyapunov1}) yields
%\begin{align}
%\dot{{V}} & \leq -(1/2)\boldsymbol\xi_p^{T}{Q_p} \boldsymbol\xi_p+  {s_p}^{T} \lbrace- c_p (s_p/||s_p||)+\boldsymbol \sigma_p \rbrace  \nonumber\\
%&-(1/2)\boldsymbol\xi_q^{T}{Q_q} \boldsymbol\xi_q+  {s_q}^{T} \lbrace-c_q (s_q/||s_q||)+\boldsymbol \sigma_q \rbrace  \nonumber\\
%&  +\sum_{i=0}^{1}{(\hat{\beta}_{ip}-\beta_{ip})\dot{\hat{\beta}}_{ip}} +{(\hat{\beta}_{iq}-\beta_{iq})\dot{\hat{\beta}}_{iq}} \nonumber %\hat{\beta}_2 || \mathbf{s}|| 
%\end{align}
%\vspace{-5mm}
\begin{align}
\dot{{V}}& \leq - (1/2)(\boldsymbol\xi_p^{T}{Q_p} \boldsymbol\xi_p+\boldsymbol\xi_q^{T}{Q_q} \boldsymbol\xi_q)- c_p || {s_p} || - c_q || {s_q} || \nonumber\\
&+ (\beta_{0p} + \beta_{1p}\boldsymbol ||\xi_p ||) || {s_p}||+(\beta_{0q}+ \beta_{1q}|| \boldsymbol \xi_q ||) || {s_q}||  \nonumber\\
& +\sum_{i=0}^{1}\lbrace(\hat{\beta}_{ip}-\beta_{ip})||\xi_p ||^i || {s_p}|| +(\hat{\beta}_{iq}-\beta_{iq})|| \boldsymbol \xi_q ||^i || {s_q}|| \rbrace \nonumber\\
& \leq -(1/2)( \lambda_{\min}(Q_p)||{\boldsymbol \xi_p}||^2+ \lambda_{\min}(Q_q)||{\boldsymbol \xi_q}||^2) \leq 0.  \label{case 1}
\end{align}
%implying that ${\bar{V}}(t) \in \mathcal{L}_{\infty}$ implying $\boldsymbol \xi_p(t), \boldsymbol \xi_q(t), \hat{\beta}_{ip}(t), \hat{\beta}_{iq}(t) \in \mathcal{L}_{\infty}$ for Case (i).

 \textbf{Case (ii):} Both $\dot{\hat{\beta}}_{ip}(t) < 0, \dot{\hat{\beta}}_{iq}(t) < 0 $ \\
For this case, following the steps as in Case (i), one has% the time derivative of (\ref{lyapunov1}) yields
\begin{align}
&\dot{V} \leq %-  (1/2)(\boldsymbol\xi_p^{T}{Q_p} \boldsymbol\xi_p+\boldsymbol\xi_q^{T}{Q_q} \boldsymbol\xi_q)- c_p || {s_p} || - c_q || {s_q} || \nonumber\\
%&+ (\beta_{0p} + \beta_{1p}\boldsymbol ||\xi_p ||) || {s_p}||+(\beta_{0q}+ \beta_{1q}|| \boldsymbol \xi_q ||) || {s_q}||  \nonumber\\
%& -\sum_{i=0}^{1}\lbrace(\hat{\beta}_{ip}-\beta_{ip}^{})||\xi_p ||^i || {s_p}|| +(\hat{\beta}_{iq}-\beta_{iq}^{})|| \boldsymbol \xi_q ||^i || {s_q}|| \rbrace \nonumber\\
 \leq -(1/2) (\lambda_{\min}(Q_p)||{\boldsymbol \xi_p}||^2 + \lambda_{\min}(Q_q)||{\boldsymbol \xi_q}||^2)\nonumber\\
&+2 \lbrace (\beta_{0p}^{}+\beta_{1p}^{}|| \boldsymbol \xi_p ||) || s_p || +(\beta_{0q}^{}+\beta_{1q}^{}|| \boldsymbol \xi_q ||) || s_q || \rbrace .\label{case 2}
\end{align}
The conditions $s_p^T \dot{s}_p \leq 0, s_q^T \dot{s}_q \leq 0$ in (\ref{ATRC_p}) and (\ref{ATRC}) yield $ || {s_p} ||, || {s_q} ||, || \boldsymbol \xi_p ||, || \boldsymbol \xi_q ||  \in \mathcal{L}_\infty$. % (cf. the relation ${s_p} =  B^T  U_p \boldsymbol \xi_p $, ${s_q} =  B^T  U_q \boldsymbol \xi_q $). 
Thus, $\exists \varsigma_p, \varsigma_q  \in \mathbb{R}^{+}$ such that $$2 (\beta_{0p}^{}+\beta_{1p}^{}|| \boldsymbol \xi_p ||) || s_p || \leq \varsigma_p , ~2 (\beta_{0q}^{}+\beta_{1q}^{}|| \boldsymbol \xi_q ||) || s_q || \leq \varsigma_q. $$ 
The fact that $\hat{\beta}_{ip}, \hat{\beta}_{iq} \in \mathcal{L}_{\infty}$ in Case (i) and decrease in Case (ii) implies $\exists \varpi_p, \varpi_q \in \mathbb{R}^{+}$ such that $\sum_{i=0}^{1}{(\hat{\beta}_{ip}-\beta_{ip}^{})^2} \leq \varpi_p, ~\sum_{i=0}^{1}{(\hat{\beta}_{iq}-\beta_{iq}^{})^2} \leq \varpi_q$. Therefore, from (\ref{lyapunov1}) we have
\begin{equation}
{V} \leq   \lambda_{\max} ({U_p}) ||{\boldsymbol \xi_p}||^2+ \lambda_{\max} ({U_q}) ||{\boldsymbol \xi_q}||^2 + \varpi_p+\varpi_q. \label{V}
\end{equation}
Using the relation (\ref{V}), (\ref{case 2}) can be written as
\begin{equation}
\dot{V} \leq - \upsilon V  + \varsigma_p+  \varsigma_q + \upsilon (\varpi_p+\varpi_q), \label{V_dot}
\end{equation}
where $\upsilon \triangleq \frac{\min \lbrace  \lambda_{\min}(Q_p),  \lambda_{\min}(Q_q) \rbrace}{\max \lbrace \lambda_{\max} ({U_p}), \lambda_{\max} ({U_q})  \rbrace}$. %Hence, $\dot{\bar{V_p}} <0$  would be achieved when $||{\boldsymbol \xi_p}|| \geq \sqrt{({\varsigma+ \upsilon \varpi_p})/{z}} $. % and the system would be UUB. 


\par \textbf{Case (iii):}  $\dot{\hat{\beta}}_{ip}(t) > 0, \dot{\hat{\beta}}_{iq}(t) < 0 $ \\
Following the derivations for Cases (i) and (ii) we have
\begin{align}
\dot{V} &\leq -(1/2) (\lambda_{\min}(Q_p)||{\boldsymbol \xi_p}||^2 + \lambda_{\min}(Q_q)||{\boldsymbol \xi_q}||^2)
+2 (\beta_{0q}^{}+\beta_{1q}^{}|| \boldsymbol \xi_q ||) || s_q ||  \leq  - \upsilon V  +  \varsigma_q + \upsilon \varpi_q. \label{case 3}
\end{align}
\textbf{Case (iv):} $\dot{\hat{\beta}}_{ip}(t) < 0, \dot{\hat{\beta}}_{iq}(t) > 0 $ \\
Following the previous cases yields
\begin{align}
\dot{V} &\leq -(1/2) (\lambda_{\min}(Q_p)||{\boldsymbol \xi_p}||^2 + \lambda_{\min}(Q_q)||{\boldsymbol \xi_q}||^2)+2 (\beta_{0p}^{}+\beta_{1p}^{}|| \boldsymbol \xi_p ||) || s_p ||   \leq  - \upsilon V  +  \varsigma_p + \upsilon \varpi_p.\label{case 4}
\end{align}
The stability results from Cases (i)-(iv) reveal that the closed-loop system is UUB.




\section{Experimental Results and Analysis}
The proposed ARTDE is tested on a quadrotor setup (Q-450 frame, Turnigy SK3-2826 motors, approx. $1.4$ kg excluding accessories and payload) which uses Raspberry Pi-4 as a processing unit and one electromagnetic gripper (0.03 kg approx. $0.03$ kg). %Excluding the processing unit, gripper and any payload, the quadrotor weighs approx. $1.4$ kg. 
Optitrack motion capture system (at 60fps) and IMU data were used to obtain the necessary state and state-derivatives feedback. %The gripper operation is not related to the control design and is operated via a remote signal. 
To properly verify the importance of the proposed controller, ARTDE is compared with a conventional adaptive TDE (ATDE) \cite{lee2019adaptive}, and also with a non-TDE adaptive method, adaptive sliding mode control (ASMC) \cite{mofid2018adaptive}. %ARTDE mainly differs from ATDE and ASMC in the way its switching gain is adapted to tackle state-dependent uncertainty and the consequent stability analysis. % of [29] relies on the TDE error being a priori bounded

\subsubsection{Experimental Scenario and Parameter Selection}
 The objective is the quadrotor should follow an infinity-shaped 2-loop path in 3D plane (cf. Fig. \ref{fig:3D_Traj}); the height from the ground is purposefully kept relatively small, as it is well-known that near-ground operations are more challenging to control since unknown ground-reaction forces are created by displaced wind from propellers. In addition, a fan is used to create external wind disturbances. The experimental scenario consists of the following sequences (cf. Fig. \ref{fig:stages}): 
\begin{itemize}
    \item The quadrotor starts from the center of the path (where the loops intersect) with a payload ($0.35$kg), it completes one loop with the payload and drops it at its starting position ($t=35$s).
    \item Then, the quadrotor completes another loop without the payload and comes back to the origin.
\end{itemize}
The gripper is operated via a remote signal, which is separate from the proposed control design. For experiment, the control parameters of the proposed ARTDE are selected as: $\bar{ m}=1$ kg, $\bar{J}=0.015I$ (kgm$^2$), ${K}_{2p}=K_{2q} =10$, $  K_{1p}=K_{1q}=5$, $L=0.015$,
${Q_p=Q_q =I}$, $\epsilon_p=\epsilon_q=5\times10^{-5}$, $\underline{\beta}_{ip}=\underline{\beta}_{iq}=0.01$, $\hat{\beta}_{ip}(0)=\hat{\beta}_{iq}(0)=0.01$, $i=0,1$. {For parity in comparison, same values of $\bar{ m}, \bar{J}$, ${K}_{ip},K_{iq}$ and $L=1/60$ are selected for ATDE \cite{lee2019adaptive}}, sliding variables for ASMC \cite{mofid2018adaptive} are selected to be $s_p$ and $s_q$. Other control parameters for ATDE and ASMC are as per \cite{lee2019adaptive} and \cite{mofid2018adaptive}, respectively.

\begin{figure}[!h]
    \includegraphics[width=3.5in, height= 3.5in]{images/quadrotor/3d_plot.png}
    \centering
    \caption{Tracking performance of the Infinity-shaped loop.}
    \label{fig:3D_Traj}
\end{figure}
\begin{figure}[!h]
    \includegraphics[width=3.5in, height= 3.5in]{images/quadrotor/3d_plot_xz_plane.png}
    \centering
    \caption{Tracking performance of the Infinity-shaped loop in XZ Plane.}
    \label{fig:3D_Traj}
\end{figure}
\begin{figure}[!h]
    \includegraphics[width=3.5in, height= 3.5in]{images/quadrotor/3d_plot_yz_plane.png}
    \centering
    \caption{Tracking performance of the Infinity-shaped loop in YZ Plane.}
    \label{fig:3D_Traj}
\end{figure}
\begin{figure}[!h]
    \includegraphics[width=\linewidth]{images/quadrotor/Inf_Fan_att_error_new.png}
    \centering
    \caption{Attitude tracking error comparison.}
    \label{fig:error_att_exp1}
\end{figure}


\begin{figure}[!h]
    \includegraphics[width=\linewidth]{images/quadrotor/Inf_Fan_pos_error_new.png}
\centering
    \caption{Position tracking error comparison.}
    \label{fig:error_exp1}
\end{figure}


\subsubsection{Experimental Results and Analysis} The performances of the controllers are compared via Figs. \ref{fig:error_exp1}-\ref{fig:error_att_exp1} and via Table \ref{table 1} in terms of root-mean-squared (RMS) error and peak error (absolute value). The error plots reveal that both ATDE and ASMC show turbulent behaviour while following the trajectory, specifically in the $y$ direction. The quadrotor also swayed after dropping the payload, while the proposed ARTDE could maintain its position after dropping of payload. This can be verified from Table \ref{table 1}, where ARTDE provides more than $30\%$ improved accuracy compared to ATDE and ASMC in $y$ and $z$ directions. These results clearly show the benefit of considering state-dependent error-based adaptive control law as opposed to the conventional a priori bounded adaptive control structures. %The attitude error comparison as seen is Table \ref{table 1} shows the stability of flight of the quadrotor with the proposed controller(ARDTC) 


% ($14.9 \%$) , 24.6% 23.6% 
 %various position Though the sliding mode controller is stable, it also shows a drop in the altitude after the payload is loaded, whereas the altitude trajectory followed by the drone with the proposed controller so similar for both loaded and unloaded cases.

% \begin{figure}[!h]
%     \includegraphics[width=1.1\columnwidth]{pos_track_inf_fan.png}
%     \centering
%     \caption{Position tracking comparison for infinity shaped payload manoeuvre}
%     \label{fig:traj_exp1}
% \end{figure}



%\begin{figure}[!h]
%    \includegraphics[width=3.5in, height= 2.5in]{3d_plot_xz_plane.png}
%    \centering
%    \caption{Tracking performance of the Infinity-shaped loop in XZ Plane.}
%    \label{fig:3D_Traj}
%\end{figure}
%\begin{figure}[!h]
%    \includegraphics[width=3.5in, height= 2.5in]{3d_plot_yz_plane.png}
%    \centering
%    \caption{Tracking performance of the Infinity-shaped loop in YZ Plane.}
%    \label{fig:3D_Traj}
%\end{figure}

\vspace{-2mm}

\begin{table}[!h]
\renewcommand{\arraystretch}{1.0}
\caption{{Performance comparison}}
\vspace{-1mm}
\label{table 1}
		\centering
{
{	\begin{tabular}{c c c c c c c}
		\hline
		\hline
		& \multicolumn{3}{c}{RMS error (m)} & \multicolumn{3}{c}{RMS error (degree)}  \\ \cline{1-7}
		 Controller & $x$ & $y$  & $z$  & $\phi$ & $\theta$  & $\psi$  \\
		 \hline
		ATDE \cite{lee2019adaptive} & 0.07& 0.15  & 0.13 & 3.37 & 2.28  & 2.22 \\
		\hline
		
		ASMC \cite{mofid2018adaptive}& 0.07 & 0.13 & 0.13 & 2.04 & 1.81 & 2.46 \\
		\hline
		ARTDE (proposed)& { 0.06} & { 0.10}  & {0.04} & 2.12 & 1.72  & 2.50 \\
		\hline
		\hline
		& \multicolumn{3}{c}{Peak error (m)} & \multicolumn{3}{c}{Peak error (degree)}  \\ \cline{1-7}
		 Controller & $x$ & $y$  & $z$  & $\phi$ & $\theta$  & $\psi$  \\
		 \hline
		ATDE \cite{lee2019adaptive} & 0.09 & 0.27  & 0.27 & 15.32 & 8.29  & 6.01 \\
		\hline
		
		ASMC \cite{mofid2018adaptive} & 0.13 & 0.25 & 0.25 & 9.53 & 6.46 & 7.50 \\
		\hline
		ARTDE (proposed)& { 0.09} & { 0.22}  & {0.25} & 7.46 & 6.25  & 5.76 \\
		\hline
		\hline
\end{tabular}}}
\end{table}
